Sentence Object Notation: Multilingual sentence notation based on Wordnet

The representation of sentences is a very important task. It can be used as a way to exchange data inter-applications. One main characteristic, that a notation must have, is a minimal size and a representative form. This can reduce the transfer time, and hopefully the processing time as well. Usually, sentence representation is associated to the processed language. The grammar of this language affects how we represent the sentence. To avoid language-dependent notations, we have to come up with a new representation which don't use words, but their meanings. This can be done using a lexicon like wordnet, instead of words we use their synsets. As for syntactic relations, they have to be universal as much as possible. Our new notation is called STON "SenTences Object Notation", which somehow has similarities to JSON. It is meant to be minimal, representative and language-independent syntactic representation. Also, we want it to be readable and easy to be created. This simplifies developing simple automatic generators and creating test banks manually. Its benefit is to be used as a medium between different parts of applications like: text summarization, language translation, etc. The notation is based on 4 languages: Arabic, English, Franch and Japanese; and there are some cases where these languages don't agree on one representation. Also, given the diversity of grammatical structure of different world languages, this annotation may fail for some languages which allows more future improvements.

==> Codes/comp-eg2.tex <==
\begin{minipage}{0.45\textwidth}
%\begin{multicols}{2}
\begin{verbatim}
	@act:[
	   act:{
	      id: represent;
	      syn: 988028;
	      tns: PR;
	      agt: [karim];
	      thm: [sentence];
	   act:}
	   act:{
	      id: hope;
	      syn: 1811441;
	      tns: PR;
	      agt: [karim];
	      thm: [represent];
	   act:}
	act:]
\end{verbatim}
%\end{multicols} 
\end{minipage}

==> Codes/graf.tex <==
\begin{minipage}{.97\textwidth}
%\begin{multicols}{2}
\begin{verbatim}
	<node xml:id="tml-n1"/>
	<a label="EVENT" ref="tml-n1" as="TimeML">
	   <fs>
	      <f name="event" value="fast"/>
	      <f name="tense" value="Past"/>
	      <f name="signature" value="individual"/>
	   </fs>
	</a>
	<edge xml:id="tml-e1" from="tml-n1" to="t2"/>
	<node xml:id="tml-n2"/>
	<a label="TIME-AMOUNT" ref="tml-n2" as="TimeML">
	   <fs>
	      <f name="numeral" value="2"/>
	      <f name="unit" value="day"/>
	   </fs>
	</a>
	<edge xml:id="tml-e2" from="tml-n2" to="t4"/>
	<edge xml:id="tml-e3" from="tml-n2" to="t5"/>
	<edge xml:id="tml-e4" from="tml-n1" to="tml-n2"/>
	<a label="MLINK" ref="tml-e4" as="TimeML">
	   <fs>
	      <f name="relType" value="FOR"/>
	   </fs>
	</a>
\end{verbatim}
%\end{multicols}
\end{minipage} \\
Tokens: [I$_{t1}$] [fasted$_{t2}$] [for$_{t3}$] [two$_{t4}$] [days$_{t5}$].

==> Codes/lopatkova.tex <==
\begin{minipage}{.97\textwidth}
\begin{tabular}{lll}
\{ [Klejch]0 & \b{,} \{ [kter\'{y} dal dev\v{e}t ze dvan\'{a}cti g\'{o}l\r{u} Zl\'{\i}na]1 \}1 \b{,} & [m\'{a} vydatn\'{e} pomocn\'{\i}ky]0 \}1 \b{.}\\
Klejch & who scored nine out twelve goals for Zl\'{\i}n & has good helpers . \\
\end{tabular}
\end{minipage}

==> Codes/ston-sem.back.tex <==
\begin{minipage}{0.97\textwidth}
\begin{multicols}{3}
\begin{verbatim}
@r:[
  r:{
    id: soldier;
    syn: 10622053;
    def: Y
  r:}
  r:{
    id: battle;
    syn: 953559
  r:}
  r:{
    id: fear;
    syn: 7519253;
    def: N
  r:}
  r:{
    id: afraid-soldier;
    syn: 10622053;
    @adj:[
      adj:{
        syn: 77645
      adj:}
    adj:]
  r:}
r:]

@act:[
  act:{
    id: was;
    syn: 2604760;
    tns: PA;
    agt: [soldier];
    thm: [afraid-soldier];
    @rel:[
      rel:{
        typ: OF;
        ref: [battle];
      rel:}
    rel:]
  act:}
  act:{
    id: feared;
    syn: 1780729;
    tns: PA;
    agt: [soldier];
    thm: [battle];
  act:}
  act:{
    id: had;
    syn: 121046;
    tns: PA;
    agt: [soldier];
    thm: [fear];
    @rel:[
      rel:{
        typ: OF;
        ref: [battle];
      rel:}
    rel:]
  act:}
act:]
@st:[
  st:{
    typ: AFF;
    act: [was]
  st:}
  st:{
    typ: AFF;
    act: [feared]
  st:}
  st:{
    typ: AFF;
    act: [had]
  st:}
st:]
\end{verbatim}
\end{multicols} 
\end{minipage}

==> Codes/unl2.tex <==
\begin{minipage}{.97\textwidth}
%\begin{multicols}{2}
\begin{verbatim}
{unl}
   agt(go(icl>move>do,plt>place,plf>place,agt>thing)
     .@entry.@past,i(icl>person))
     
   plt(go(icl>move>do,plt>place,plf>place,agt>thing)
     .@entry.@past,malaysia(iof>asian_country>thing))
     
   plf(go(icl>move>do,plt>place,plf>place,agt>thing)
     .@entry.@past,bangladesh(iof>asian_country>thing))
     
   met(go(icl>move>do,plt>place,plf>place,agt>thing)
     .@entry.@past,aeroplane(icl>heavier-than-air_craft>thing, 
       equ>airplane))
     
   obj:01(attend(icl>go_to>do,agt>person,obj>place)
     .@entry,conference(icl>meeting>thing).@indef)
     
   pur(go(icl>move>do,plt>place,plf>place,agt>thing)
     .@entry.@past,:01)
{/unl}
\end{verbatim}
%\end{multicols}
\end{minipage}\\
I went to Malaysia from Bangladesh by aeroplane to attend a conference


==> Tables/cmp-eg.back.tex <==
\begin{tabular}{ll}
\hline\noalign{\smallskip}
Language & Sentence \\
\noalign{\smallskip}\hline\noalign{\smallskip}

Arabic & \RL{kariym 'a.twalu min" 'axiyh.} \\
& /Kar\={\i}m a\d{t}walu min akh\={\i}h./  \\
& \RL{kariym yusaA`idu 'aqalla min" 'axiyh.} \\
& /Kar\={\i}m yus\={a}`idu aqalla min akh\={\i}h./  \\

English & Karim is taller than his brother. \\
& Karim helps less than his brother. \\

French & Karim est plus grand que son frère. \\
& Karim aide moins que son frère. \\

Japanese & \JP{カリムさんは兄弟より背が高いです。} \\
& /Karimu-san wa ky\={o}dai yori se ga takai desu./ \\
& \JP{カリムさんは兄弟より手伝うのが少ないです。} \\
& /Karimu-san wa ky\={o}dai yori tetsudau no ga sukunai desu./ \\

\hline\noalign{\smallskip}
\end{tabular} 


==> Tables/cmp-eg.back2.tex <==
\begin{tabular}{lll}
\hline\noalign{\smallskip}
Language & Sentence 1 & Sentence 2 \\
\noalign{\smallskip}\hline\noalign{\smallskip}

Arabic & \RL{kariym 'a.twalu min" 'axiyh.} & \RL{kariym yusaA`idu 'aqalla min" 'axiyh.} \\
& /Kar\={\i}m a\d{t}walu min akh\={\i}h./  & /Kar\={\i}m yus\={a}`idu aqalla min akh\={\i}h./\\
\noalign{\smallskip}

English & Karim is taller than his brother. & Karim helps less than his brother.\\
\noalign{\smallskip}

French & Karim est plus grand que son frère. & Karim aide moins que son frère. \\
\noalign{\smallskip}

Japanese & \JP{カリムさんは兄弟より背が高いです。} & \JP{カリムさんは兄弟より手伝うのが少ないです。} \\
& /Karimu-san wa ky\={o}dai yori se ga takai desu./ & /Karimu-san wa ky\={o}dai yori tetsudau no ga sukunai desu./ \\

\hline\noalign{\smallskip}
\end{tabular} 


==> Tables/hungry-past.tex <==
\begin{tabular}{ll}
\hline\noalign{\smallskip}
Language & Sentence \\
\noalign{\smallskip}\hline\noalign{\smallskip}
Arabic & \RL{'anA jaw`aAn.} \\
& /an\={a} jaw`\={a}n./ \\
English & I am hungry. \\
French & J'ai faim. \\
Japanese & \JP{お腹が空いた。} \\
& /onaka ga suita./ \\
\noalign{\smallskip}\hline
\end{tabular}
